When Deepfake Detection Meets Graph Neural Network:a Unified and Lightweight Learning Framework

The proliferation of generative video models has made detecting AI-generated and manipulated videos an urgent challenge. Existing detection approaches often fail to generalize across diverse manipulation types due to their reliance on isolated spatial, temporal, or spectral information, and typically require large models to perform well. This paper introduces SSTGNN, a lightweight Spatial-Spectral-Temporal Graph Neural Network framework that represents videos as structured graphs, enabling joint reasoning over spatial inconsistencies, temporal artifacts, and spectral distortions. SSTGNN incorporates learnable spectral filters and spatial-temporal differential modeling into a unified graph-based architecture, capturing subtle manipulation traces more effectively. Extensive experiments on diverse benchmark datasets demonstrate that SSTGNN not only achieves superior performance in both in-domain and cross-domain settings, but also offers strong efficiency and resource allocation. Remarkably, SSTGNN accomplishes these results with up to 42$\times$ fewer parameters than state-of-the-art models, making it highly lightweight and resource-friendly for real-world deployment.

==> floats/fig_patch_size.tex <==
\begin{figure}[!t]
  \centering
  %\vspace{0.2cm}
\includegraphics[width=1\linewidth]{Figure_1.pdf}
  \vspace{-0.2cm}
  \caption{Ablation: patch size and graph thresholds $\tau$.}
  \label{abla2}
\end{figure}

==> floats/fig_tsne_old.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.23\textwidth]{Figure_4-1.pdf}
    \includegraphics[width=0.23\textwidth]{Figure_4-2.pdf}
\vspace{-0.2cm}
\caption{t-SNE visualization of the learned features from (a) STIL and (b) \ourmethod{} on FF++. We highlight that \ourmethod{} achieves a more natural separation between real and fake samples, demonstrating improved generalization to unseens.}%, compared to STIL which exhibits stronger fake pattern domination and less clear boundary distinctions.}
\label{vaoss}
\end{figure}

==> floats/tab_corss_1-1_FF.tex <==
\begin{comment}

\begin{table}[!t]
\small
\centering
\caption{Cross-domain: 1-to-1 setting from FF+ to others.\haoyu{to appendix.}}
\setlength{\tabcolsep}{7pt}
\renewcommand{\arraystretch}{1.}
\begin{tabular}{l|c|c|c}
\toprule
\textbf{Methods} & \textbf{Wild-DF} & \textbf{CD-v2} & \textbf{DFDC} \\
\midrule
Xception   & 62.72 & 61.80 & 63.61 \\
MultiAtt   & 59.74 & 67.02 & 68.01 \\
RECCE      & 64.31 & 68.71 & 69.06 \\
DCL        & {\color{blue}\textbf{71.14}} & {\color{blue}\textbf{82.30}} & {\color{blue}\textbf{76.71}} \\ \midrule
\textbf{\ourmethod{}}     & {\color{red}\textbf{75.31}} & {\color{red}\textbf{83.45}} & {\color{red}\textbf{79.26}} \\
\bottomrule
\end{tabular}
\label{cross2}
\end{table}

\mypara{1-to-1 setting.}  
Building upon the cross-type generalization results within FF++, we further assess the cross-dataset generalization abil  ity of each method by training on the full FF+ dataset and testing on three challenging and diverse benchmarks: Wild-DF, CD-v2, and DFDC (Table~\ref{cross2}). Once again, our method demonstrates superior generalization capability, achieving the highest accuracy across all three datasets: 75.31\% on Wild-DF, 83.45\% on CD-v2, and 79.26\% on DFDC, outperforming all baselines. DCL performs second best, with 71.14\%, 82.30\%, and 76.71\% on the respective datasets, while previous methods such as Xception and MultiAtt lag significantly behind.  
It is worth noting that Wild-DF and DFDC represent unconstrained, real-world video conditions with greater variation in lighting, compression, and spoofing artifacts. Our method’s strong performance in these settings underscores its practical robustness and ability to generalize to previously unseen domains.
\end{comment}

\begin{table}[!t]
\small
\centering
\caption{Cross-domain: 1-to-3 setting from training on \textit{SVD} and testing on \textit{Crafter}, \textit{Gen2} and \textit{Lavie}.}
\setlength{\tabcolsep}{6.2pt}
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{l|cc|cc|cc}
\toprule
\multirow{2}{*}{\textbf{Methods}} 
    & \multicolumn{2}{c|}{\textbf{Crafter}} 
    & \multicolumn{2}{c|}{\textbf{Gen2}}
    & \multicolumn{2}{c}{\textbf{Lavie}}
     \\
     \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
 & Acc & AUC & Acc & AUC & Acc & AUC \\
\midrule
STIL & \textbf{\textcolor{red}{96.89}} & 99.75 & \textbf{\textcolor{blue}{93.12}} & 96.84 & 92.04 & \textbf{\textcolor{red}{97.10}} \\
DCL & 93.46 & 99.43 & 92.65 & \textbf{\textcolor{red}{99.10}} & 89.72 & 95.31 \\
MINTIME & 89.25 & 94.14 & 88.10 & 94.75 & 84.25 & 91.34 \\
TALL & \textbf{\textcolor{blue}{95.14}} & 97.93 & 88.74 & 87.61 & 84.30 & 81.33\\
\midrule
\textbf{\ourmethod{}} & 94.77 & \textbf{\textcolor{red}{99.96}} & \textbf{\textcolor{red}{95.31}} & \textbf{\textcolor{blue}{98.98}} & \textbf{\textcolor{red}{92.90}} & \textbf{\textcolor{blue}{96.35}} \\
\bottomrule
\end{tabular}
\label{tab:cross4}
\end{table}

